Seeing Around Corners with Edge-Resolved Transient Imaging

Non-line-of-sight (NLOS) imaging is a rapidly growing field seeking to form images of objects outside the field of view, with potential applications in search and rescue, reconnaissance, and even medical imaging. The critical challenge of NLOS imaging is that diffuse reflections scatter light in all directions, resulting in weak signals and a loss of directional information. To address this problem, we propose a method for seeing around corners that derives angular resolution from vertical edges and longitudinal resolution from the temporal response to a pulsed light source. We introduce an acquisition strategy, scene response model, and reconstruction algorithm that enable the formation of 2.5-dimensional representations -- a plan view plus heights -- and a 180$^{\circ}$ field of view (FOV) for large-scale scenes. Our experiments demonstrate accurate reconstructions of hidden rooms up to 3 meters in each dimension.

==> SuppSubfiles/notation.tex <==

\newcommand{\CS}[1]{\color{green}{#1}} % For comments
\newcommand{\Frac}[2]{{{#1}/{#2}}}  % an "inert" form of \frac

% Vectors
\def\Veca{\mathbf{a}}
\def\Vecb{\mathbf{b}}
\def\Vecc{\mathbf{c}}
\def\Vecd{\mathbf{d}}
\def\Vecf{\mathbf{f}}
\def\Vecg{\mathbf{g}}
\def\Vech{\mathbf{h}}
\def\Veck{\mathbf{k}}
\def\Vecl{\mathbf{l}}
\def\Vecm{\mathbf{m}}
\def\Vecn{\mathbf{n}}
\def\Vecp{\mathbf{p}}
\def\Vecq{\mathbf{q}}
\def\Vecr{\mathbf{r}}
\def\Vecs{\mathbf{s}}
\def\Vecu{\mathbf{u}}
\def\Vecv{\mathbf{v}}
\def\Vecw{\mathbf{w}}
\def\Vecx{\mathbf{x}}
\def\Vecy{\mathbf{y}}
\def\Vecz{\mathbf{z}}

\def\Veckap{\bm{\kappa}}
\def\Vecphi{\bm{\phi}}

\def\Vecytheta{\mathbf{y}_{\theta}}

\def\Diffy{\mathbf{y}}
\def\NMeas{\Vecm}

% Matrices
\def\VecA{\mathbf{A}}
\def\VecB{\mathbf{B}}
\def\VecC{\mathbf{C}}
\def\VecD{\mathbf{D}}
\def\VecE{\mathbf{E}}
\def\VecF{\mathbf{F}}
\def\VecG{\mathbf{G}}
\def\VecI{\mathbf{I}}
\def\VecJ{\mathbf{J}}
\def\VecK{\mathbf{K}}
\def\VecH{\mathbf{H}}
\def\VecM{\mathbf{M}}
\def\VecP{\mathbf{P}}
\def\VecR{\mathbf{R}}
\def\VecS{\mathbf{S}}
\def\VecT{\mathbf{T}}
\def\VecU{\mathbf{U}}
\def\VecV{\mathbf{V}}
\def\VecW{\mathbf{W}}
\def\VecX{\mathbf{X}}
\def\VecY{\mathbf{Y}}
\def\VecZ{\mathbf{Z}}


\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% Transpose 
\def\transpose{^{\!\mathsf{T}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\yv{\Vecy^v}
\def\yh{\Vecy^h}
\def\Vecups{\bm{\upsilon}}
\def\fr{f_{\rm r}}
\def\nb{n_b}
\def\nl{n_\ell}
\def\rl{r_\ell}
\def\ro{r_o}
\def\rs{r_s}
\def\tbin{t_{\rm bin}}
\def\tdw{t_{\rm dwell}}
\def\th{t_{\rm h}}
\def\tr{t_{\rm r}}
\def\pcloud{\Phi}
\def\nfacets{N_{\pcloud}}
\newcommand{\intf}[1]{\alpha_{#1}}
\newcommand{\hf}[1]{\eta_{#1}}
\newcommand{\af}[1]{\phi_{#1}}
\newcommand{\tintf}[1]{\tilde{\alpha}_{#1}}
\newcommand{\thf}[1]{\tilde{\eta}_{#1}}
\newcommand{\taf}[1]{\tilde{\phi}_{#1}}
\newcommand{\df}[1]{\rho_{#1}}
\newcommand{\cf}[1]{\mathbf{c}_{#1}}
\newcommand{\Hyp}{\mathbf{\Psi}}
\newcommand{\DiffY}{\mathbf{Y}}

\newcommand{\ceila}{\alphac}
\newcommand{\ceilh}{\etac}
\newcommand{\ceil}{\bm{\chi}}
\newcommand{\hatceil}{\widehat{\bm{\chi}}}

\def\bp{\bm{p}}
\def\der{\, {\rm d}}
\def\nfl{\Vecn_{\Vecell}}
\def\nfc{\Vecn_{\Vecc}}
\def\nfp{\Vecn_{\Vecp}}
\def\nff{\Vecn_{\Vecf}}
\def\nfg{\Vecn_{\Vecg}}

\def\Vecalpha{\bm{\alpha}}
\def\Veceta{\bm{\eta}}
\def\Vecell{\bm{\ell}}
\def\Vecrho{\bm{\rho}}
\def\Vecphi{\bm{\phi}}

\def\up{\Vecu_\Vecp}

\def\CalR{\mathcal{R}}
\def\CalS{\mathcal{S}}
\def\Delt{\Delta_t}
\def\Dth{\Delta_\theta}

\def\ximax{\xi_{\rm max}}
\def\ximin{\xi_{\rm min}}
\def\rmid{r_{\rm mid}}
\def\magphi{|\phi|}

\def\etac{\eta_{\rm c}}
\def\rhoc{\rho_{\rm c}}
\def\alphac{\alpha_{\rm c}}



\def\smid{\,|\,}     % Like \mid, but with less space; use for conditioning
\def\ssim{\,\sim\,}  % Make it easier to parse many expressions with \sim

